Monadic type-and-effect soundness

We introduce the abstract notions of "monadic operational semantics", a small-step semantics where computational effects are modularly modeled by a monad, and "type-and-effect system", including "effect types" whose interpretation lifts well-typedness to its monadic version. In this meta-theory, as usually done in the non-monadic case, we can express progress and subject reduction properties and provide a proof, given once and for all, that they imply soundness. The approach is illustrated on a lambda calculus with generic effects. We equip the calculus with an expressive type-and-effect system, and provide proofs of progress and subject reduction which are parametric on the interpretation of effect types. In this way, we obtain as instances many significant examples, such as checking exceptions, preventing/limiting non-determinism, constraining order/fairness of outputs on different locations. We also provide an extension with constructs to raise and handle computational effects, which can be instantiated to model different policies.

==> conf-bib-macros.tex <==

\newcommand{\APLAS}[2]{Proceedings of the #1 Asian Symposium on Programming Languages and Systems, {APLAS} #2} 

\newcommand{\CMCS}[2]{Proceedings of the #1 Workshop on Coalgebraic Methods in Computer Science, {CMCS} #2} 


\newcommand{\ECOOP}[2]{#1 European Conference on Object-Oriented Programming, {ECOOP} #2}
\newcommand{\ESOP}[2]{Programming Languages and Systems - #1 European Symposium on Programming, {ESOP} #2} 
\newcommand{\FOSSACS}[2]{Foundations of Software Science and Computation Structures, #1 International Conference, {FoSSaCS} #2}
\newcommand{\ICFP}[2]{#1 {ACM} {SIGPLAN} International Conference on Functional Programming, {ICFP} #2} 
\newcommand{\LICS}[2]{Proceedings of the #1 Annual {ACM/IEEE} Symposium on Logic in Computer Science, {LICS} #2}
\newcommand{\MFPS}[2]{The #1 Conference on Mathematical Foundations of Programming Semantics, {MFPS} #2} 
\newcommand{\POPL}[2]{Proceedings of the #1 {ACM/SIGPLAN} Symposium on Principles of Programming Languages, {POPL} #2} 
\newcommand{\OOPSLA}[2]{Proceedings of the #1 {ACM} International Conference on Object-Oriented Programming: Systems, Languages and Applications, {OOPSLA} #2}



